LIHE: Linguistic Instance-Split Hyperbolic-Euclidean Framework for Generalized Weakly-Supervised Referring Expression Comprehension

Existing Weakly-Supervised Referring Expression Comprehension (WREC) methods, while effective, are fundamentally limited by a one-to-one mapping assumption, hindering their ability to handle expressions corresponding to zero or multiple targets in realistic scenarios. To bridge this gap, we introduce the Weakly-Supervised Generalized Referring Expression Comprehension task (WGREC), a more practical paradigm that handles expressions with variable numbers of referents. However, extending WREC to WGREC presents two fundamental challenges: supervisory signal ambiguity, where weak image-level supervision is insufficient for training a model to infer the correct number and identity of referents, and semantic representation collapse, where standard Euclidean similarity forces hierarchically-related concepts into non-discriminative clusters, blurring categorical boundaries. To tackle these challenges, we propose a novel WGREC framework named Linguistic Instance-Split Hyperbolic-Euclidean (LIHE), which operates in two stages. The first stage, Referential Decoupling, predicts the number of target objects and decomposes the complex expression into simpler sub-expressions. The second stage, Referent Grounding, then localizes these sub-expressions using HEMix, our innovative hybrid similarity module that synergistically combines the precise alignment capabilities of Euclidean proximity with the hierarchical modeling strengths of hyperbolic geometry. This hybrid approach effectively prevents semantic collapse while preserving fine-grained distinctions between related concepts. Extensive experiments demonstrate LIHE establishes the first effective weakly supervised WGREC baseline on gRefCOCO and Ref-ZOM, while HEMix achieves consistent improvements on standard REC benchmarks, improving IoU@0.5 by up to 2.5\%. The code is available at https://anonymous.4open.science/r/LIHE.

==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/1_introduction.tex <==
\section{Introduction}
% Referring Expression Comprehension (REC)~\citep{mao2016generation, yu2016modeling} aims to localize objects in an image based on natural language expressions. Traditional REC tasks predominantly focus on expressions that refer to a single target. However, real-world scenarios are often more complex: a referring expression might correspond to multiple objects or no object at all. To address this gap, the Generalized Referring Expression Comprehension (GREC)~\citep{he2023grec,liu2023gres,wu20243d}  task has been proposed, extending REC by allowing expressions to describe no-target and multi-target cases, as illustrated in Fig. \ref{fig:example}. 

% Despite the growing importance of GREC, its development has been significantly constrained by the reliance on expensive and labor-intensive instance-level annotations~\citep{zhu2022seqtr, deng2023transvg}. Recent weakly supervised REC methods~\citep{jin2023refclip, luo2024apl} alleviate this by leveraging contrastive learning~\citep{contrastive} to align vision and language features without strong supervision. However, these approaches assume a single referent per expression as shown in Appendix~\ref{Appendix:LimitationsofRefCLIP}, limiting their applicability to GREC, where the number of referents is unknown. Their reliance on contrastive objectives makes it difficult to handle multi-target scenarios, highlighting the need for a more flexible and generalizable paradigm.


% Referring Expression Comprehension (REC)~\citep{mao2016generation, yu2016modeling} has traditionally relied on fully supervised training with instance-level (box) annotations, which are costly and labor-intensive~\citep{zhu2022seqtr, deng2023transvg}. In contrast, weakly supervised REC (weak REC) methods~\citep{jin2023refclip, luo2024apl} often built on contrastive learning~\citep{contrastive}, and effectively mitigate the need for box-level labels. These approaches are attracting increasing attention, and a number of recent works~\citep{jin2023refclip,luo2024apl,cheng2025weakmcn} have demonstrated strong accuracy under weak supervision.

% Referring Expression Comprehension (REC), also known as visual grounding, aims to locate target objects in images based on given natural language descriptions. As a vision-language (VL) task, REC has shown great potential in various real-world applications, such as robot navigation and image editing, thus attracting numerous research efforts recently. Despite the progress made, most REC methods typically require a large amount of object-level labels for supervised learning, resulting in high annotation costs. To address this challenge, an increasing amount of work has focused on weakly supervised REC (WREC). Among them, early works often formulated weakly supervised REC using a two-stage pipeline, which requires an expensive region proposal stage. Recently, the one-stage framework has become a popular paradigm for weakly supervised REC due to its superior efficiency. These methods typically utilize anchor features from a pre-trained one-stage detector to represent candidate objects and directly match them with text features to determine the target referent. Based on this efficient framework, contrastive-based objectives are used to achieve effective weakly supervised learning.

% Referring Expression Comprehension (REC), also known as visual grounding, aims to locate target objects in images based on natural language descriptions, demonstrating significant potential in real-world applications such as robotic navigation and image editing. However, existing REC methods require extensive object-level annotations, necessitating the development of more cost-effective alternatives. Consequently, weakly supervised REC (WREC) has emerged as a viable solution to address this annotation bottleneck. Although early WREC methods primarily adopted two-stage pipelines and demonstrated favorable performance, they suffer from computational inefficiency due to multi-step processing. To overcome these limitations, single-stage frameworks have been increasingly adopted and established as the dominant paradigm in the field owing to their superior efficiency. These methods directly utilize anchor features from pre-trained detectors for text matching and subsequently achieve more effective weakly supervised training through contrastive learning.

% Despite the effectiveness, current single-stage WREC methods are fundamentally limited by a rigid one-to-one mapping assumption, rendering them unreliable whenever an expression's referent cardinality is not singular. This limitation leads to critical failures in two common scenarios. In one-to-many cases, such as for ``Woman and man in the apron'' in  Fig.~\ref{fig:example}, their winner-takes-all mechanism is structurally incapable of locating all relevant targets, erroneously returning only a single instance. Conversely, in one-to-zero cases, like locating ``far left sitting guy'' as shown in Fig.~\ref{fig:example}, the lack of a rejection mechanism compels models to ``hallucinate'' a grounding on an irrelevant object. This inherent inability to handle variable cardinality severely limits their robustness and generalization in realistic applications. To formally address these limitations, we introduce the \textbf{G}eneralized \textbf{W}eakly Supervised \textbf{R}eferring \textbf{E}xpression \textbf{C}omprehension (GWREC) task, a more realistic paradigm designed to handle expressions corresponding to zero, one, or multiple objects. Thanks to the latest advances of Generalized Referential Expression Understanding (GREC), we can utilize its established datasets as the training and evaluation foundation for the GWREC task.

Referring Expression Comprehension (REC)~\citep{mao2016generation,yu2016modeling}, also known as visual grounding, aims to localize objects in an image based on natural language expressions. REC has shown broad application potential in fields such as robotic navigation and image editing. However, existing REC methods heavily rely on instance-level annotations, which are expensive and labor-intensive to collect~\citep{zhu2022seqtr,deng2023transvg}. To alleviate this bottleneck, Weakly-Supervised REC (WREC) has emerged as a cost-effective alternative. WREC methods eliminate the need for bounding box supervision and instead learn to align vision and language features using only image–text pairs. Early approaches~\citep{gupta2020contrastive, liu2019adaptive} typically employed two-stage pipelines, while recent single-stage frameworks~\citep{jin2023refclip,luo2024apl,cheng2025weakmcn} have become dominant due to their superior efficiency, directly matching text with anchor features from pre-trained detectors through contrastive learning~\citep{oord2018representation}.

 However, real-world scenarios are often more complex: a referring expression might correspond to multiple objects or no object at all, known as Generalized Referring Expression Comprehension (GREC)~\citep{he2023grec,liu2023gres,wu20243d}, which extends REC by allowing expressions to describe no-target and multi-target cases (shown as Fig.~\ref{fig:example}). Accordingly, in this paper, we aim to solve a new task, Weakly-Supervised Generalized Referring Expression Comprehension (WGREC).

Extending WREC to the WGREC setting poses two fundamental challenges that need to be addressed to develop effective weakly supervised methods. The first is the ambiguity of the supervisory signal, where the winner-takes-all mechanism of previous WREC methods is structurally incapable of locating all relevant targets, erroneously returning only a single instance, as shown in Fig.~\ref{fig:example}. The second is the semantic representation collapse, which arises because conventional contrastive learning methods rely on Euclidean similarity. This assumes flat, one-to-one alignments, leading to suboptimal representations in multi-referent scenarios. For instance, an expression like ``left person'' may refer to both ``left man'' and ``left woman'' as shown in Fig.~\ref{heratical}. Pulling both specific instances toward the same general anchor (“person”) in Euclidean space unintentionally forces ``man'' and ``woman'' closer together, blurring their categorical boundaries.


% However, a fundamental limitation persists: most existing weak REC methods implicitly assume a single referent per expression (see Appendix~\ref{Appendix:LimitationsofRefCLIP}), making them ill-suited for cases where no object matches the referring expression or where multiple objects satisfy it. Such scenarios are common in real-world images, as illustrated in Fig.~\ref{fig:example}. To bridge this gap, using the GREC datasets~\citep{he2023grec, liu2023gres, wu20243d}, we define the \emph{weakly supervised Generalized Referring Expression Comprehension (WGREC)} task, extending weakly supervised REC to support both no-target and multi-target cases under weak supervision. 



\begin{figure*}
    \centering
    \vspace{-4mm}
    % \setlength{\abovecaptionskip}{6pt}   % 图像与 caption 之间的距离
    % \setlength{\belowcaptionskip}{1pt}  % caption 与正文之间的距离，负值表示更紧凑
    \includegraphics[width=1.0\linewidth]{images/first2.pdf}
    \caption{Limitations of current WREC methods. The ground truth is denoted by red bounding boxes, whereas green bounding boxes denote the predictions. Current WREC methods always select only the best anchor as output, failing to handle No-target and Multi-target cases (e.g., no red bounding box and two red bounding boxes).
    }
    \label{fig:example}
    \vspace{-5mm}
\end{figure*}

% Inspired by how humans perceive and solve referring expressions~\citep{yang2024boosting}, we propose the first weakly supervised framework for the GREC task by decomposing it into a perception stage and a grounding stage. Specifically, in the perception stage, we adopt a Vision Large Language Model (VLM)~\citep{Qwen-VL,Qwen2VL,qwen2.5-VL} to decompose the input-referring expression into a numerical prediction representing the number of existing targets and multiple short phrases, each uniquely corresponding to an individual target. In the grounding stage, these generated short phrases, together with the original image, are fed into an efficient one-stage weakly supervised REC model~\citep{jin2023refclip,luo2024apl,zhao2018wa} to ground the corresponding targets.

% The core component of the one-stage weakly supervised REC model is the similarity module, measuring the similarity of visual and textual features to guide the anchor selection. Previous work merely adopts Euclidean similarity, enforcing flat one-to-one alignments that collapse hierarchical or many-to-many relations. To address it, we design a novel hybrid Hyperbolic-Euclidean similarity calculation called HEMix that integrates Euclidean and Hyperbolic similarity measures to enhance semantic alignment between vision and language modalities. While Euclidean similarity captures fine-grained local semantic proximity, Hyperbolic similarity naturally induces a global hierarchical structure among embeddings~\citep{hyptxt1s,hyptxt2s,hyplorentz,hyppoincare,hier,hypvit,hypseg1,hypseg2,hypfs,khrulkov2020hyperbolic,hypmeru}. By leveraging the complementary strengths of both spaces, this mixed objective enables the model to achieve better semantic consistency and to generalize more effectively across different referring scenarios.

%Extending WREC to the GWREC setting poses two fundamental challenges that needed to be addressed to develop effective weakly supervised methods. The first is the \textit{ambiguity of the supervisory signal}, where weak, image-level supervision is insufficient for a model to resolve ambiguities in compositional expressions and correctly determine the number and identity of multiple referents. The second is \textit{the semantic representation collapse}, which arises because conventional contrastive learning methods rely on Euclidean similarity. This assumes flat, one-to-one alignments, leading to suboptimal representations in multi-referent scenarios. For instance, an expression like ``left person'' may refer to both ``left man'' and ``left woman''. Pulling both specific instances toward the same general anchor (``person'') in Euclidean space unintentionally forces ``man'' and ``woman'' closer together, blurring their categorical boundaries.

To address these challenges, we propose a two-stage \textbf{L}inguistic \textbf{I}nstance-Split \textbf{H}yperbolic-\textbf{E}uclidean (LIHE) framework designed to effectively localize a variable number of objects from a single expression. First, in the \textbf{Referential Decoupling} stage, LIHE leverage a vision-language model (VLM)~\citep{Qwen-VL,Qwen2VL,qwen2.5-VL} to infer the number of referring objects: if zero, it will skip the second stage; otherwise, it will decompose the expression into corresponding sub-expressions for each object. Second, the \textbf{Referent Grounding} stage employs a contrastive learning paradigm to train the model to localize each sub-expression. To prevent the semantic collapse inherent in this grounding process, LIHE integrates \textit{HEMix}, a hybrid similarity module that replaces the standard Euclidean metric. HEMix synergizes the fine-grained alignment of Euclidean proximity with the structure-preserving properties of hyperbolic geometry~\citep{ganea2018hyperbolic,hier,bdeir2024fully}. It leverages the inherent capacity of Lorentzian hyperbolic space to model hierarchies by placing general concepts near the origin and specific instances outward, thereby preserving semantic distinctions. This design, which serves as a \textit{plug-and-play} module, effectively prevents concept collapse and enhances generalization in complex referring scenarios with negligible computational overhead.


% To tackle these challenges, we propose \textbf{LIHE (Linguistic Instance-Split Hyperbolic-Euclidean)}, a two-stage framework inspired by how humans interpret and localize multiple referents from a single expression~\citep{yang2024boosting}. In the first stage, \textbf{Referential Decoupling}, we leverage vision-language models (VLMs)~\citep{Qwen-VL,Qwen2VL,qwen2.5-VL} to decompose complex expressions into semantically coherent sub-expressions. Although VLMs excel at parsing language in visual context, they lack precise grounding capabilities due to being trained on coarse-grained image-text pairs without object-level alignment. In the second stage, \textbf{Referent Grounding}, each sub-expression is localized using weak supervision. Existing contrastive learning approaches~\citep{jin2023refclip, luo2024apl} typically rely on Euclidean similarity, which assumes flat, one-to-one alignments between vision and language. This assumption often leads to suboptimal representations in multi-referent scenarios. For example, as illustrated in Fig.~\ref{heratical}(a), the expression \textit{`left person'} may refer to both \textit{`left man'} and \textit{`left woman'} in the image. Pulling both toward the same anchor unintentionally brings \textit{`man'} and \textit{`woman'} closer in the embedding space, blurring categorical boundaries and reducing discriminability. In contrast, Lorentzian hyperbolic space~\citep{hyptxt1s,hyptxt2s,hyplorentz,hyppoincare,hier,hypvit,hypseg1,hypseg2,hypfs,khrulkov2020hyperbolic,hypmeru} naturally models hierarchical relationships: general concepts are located near the origin, while more specific instances expand outward, maintaining angular separation between sibling nodes. Motivated by this property, we introduce \textit{a plug-in-play \textbf{HEMix}, which is a hybrid similarity that replaces Euclidean similarity in contrastive learning and improves any cross-entropy-based weakly supervised method relying on similarity computations with negligible additional computational overhead}. Specifically, HEMix combines Euclidean proximity for fine-grained alignment with hyperbolic geometry to preserve global semantic structure, enabling better generalization and more discriminative grounding in complex referring scenarios.

We conduct extensive experiments on the GREC datasets gRefCOCO~\citep{he2023grec} and Ref-ZOM~\citep{hu2023beyond}, demonstrating that our method is the first weakly supervised framework to tackle the WGREC task effectively. Additionally, we validate the broader applicability of HEMix on REC benchmarks, including RefCOCO~\citep{nagaraja2016modeling}, RefCOCO+~\citep{nagaraja2016modeling}, and RefCOCOg~\citep{mao2016generation}, and achieve the state-of-the-art performance. Our findings highlight the potential of combining REC with structured geometry to advance vision-language understanding.



% Our contributions can be summarized as follows:
% \begin{itemize} [leftmargin=*]
% \item We propose the first weakly supervised framework for GREC, consisting of a perception stage that predicts the number of targets and generates short, distinct phrases for each target, followed by a grounding stage that localizes targets using an efficient one-stage REC model.
% \item We introduce a novel hybrid Hyperbolic-Euclidean mix similarity (HEMix) that combines Euclidean and Hyperbolic similarities to preserve local semantic proximity while capturing global hierarchical structures, enhancing the model performance.
% \item We conduct extensive experiments on gRefCOCO, demonstrating the effectiveness of our method as the first weakly supervised approach for GREC. Furthermore, we achieve state-of-the-art performance on REC benchmarks, i.e. RefCOCO, RefCOCO+, and RefCOCOg.
% \end{itemize}

==> sections/2_related_work.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    Related Work    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Related Work}
% \paragraph{Generalized Referring Expression Comprehension}
% GREC~\citep{he2023grec} extends traditional REC tasks by permitting linguistic expressions to refer simultaneously to multiple target objects. Baseline methods such as MCN \citep{luo2020multi}, VLT \citep{ding2021vision}, MDETR \citep{kamath2021mdetr}, and UNINEXT \citep{yan2023universal} have been adopted to evaluate performance under this more complex and realistic scenario. Recent advancements include RECANTFormer \citep{hemanthage2024recantformer}, which employs a recursive transformer decoder with adaptive prediction heads to dynamically predict multiple targets, and HieA2G \citep{wang2025hierarchical}, which leverages a hierarchical alignment mechanism to enhance interactions between linguistic phrases and visual objects, thereby capturing fine-grained semantic correlations. However, these methods uniformly rely on fully supervised bounding box annotations. Weakly supervised approaches for GREC remain unexplored, motivating the development of our proposed weakly supervised framework.
% \paragraph{Weakly Supervised REC}
% Weakly supervised approaches~\citep{gupta2020contrastive,liu2019adaptive,liu2019kpnet,
% liu2021rir,sun2021discriminative,wang2021ckd,zhang2020counterfactual} have recently shown promising results in Referring Expression Comprehension (REC), significantly reducing the dependence on expensive bounding box annotations. Unlike fully supervised methods~\citep{deng2021transvg,ho2022yoro,hong2019ltrs,huang2021look,
% kamath2021mdetr,liao2020cmcf,liu2019nmtree,liu2019erase,crossdiff,
% luo2020multi,sun2021iterative,yang2019fast,yang2020recursive,
% zhang2018vc,zhao2022word2pix,zhou2021ginet,zhou2021trar,
% zhu2022seqtr}, weakly supervised REC techniques utilize coarser supervision signals, such as image-level or image-text pair annotations, enabling scalable and cost-effective training. Notable one-stage methods~\citep{jin2023refclip,luo2024apl,zhao2018wa}
% include RefCLIP \citep{jin2023refclip}, which redefines REC as an anchor-text matching task using anchor-based contrastive learning to align visual and textual features without bounding boxes, and APL \citep{luo2024apl}, which enriches anchor features through position, color, and category prompts, coupled with auxiliary losses to enhance vision-language alignment. Despite their effectiveness in traditional REC tasks, these methods inherently assume a single-target scenario, limiting their generalizability to multi-target GREC settings. This highlights the need to develop specialized, weakly supervised approaches tailored specifically to GREC.
% \paragraph{Hyperbolic Representation learning }
% Hyperbolic representation learning~\citep{hyptxt1s,hyptxt2s,hyplorentz,hyppoincare,hier,hypvit,
% hypseg1,hypseg2,hypfs,khrulkov2020hyperbolic,hypmeru} leverages hyperbolic geometry's exponential volume growth and negative curvature, making it particularly effective for modeling hierarchical and relational structures. Early seminal works such as Poincaré Embeddings \citep{nickel2017poincare} and Hyperbolic Neural Networks \citep{ganea2018hyperbolic} established foundational techniques for embedding structured data into hyperbolic spaces. Recent developments have adapted hyperbolic geometry to vision and cross-modal tasks. For instance, hyperbolic embedding methods introduced by Kwon et al.~\citep{kwon2024improving} and Kong et al.~\citep{kong2024hyperbolic} have improved visual recognition and open-world detection by preserving hierarchical semantics. For vision-language alignment, Ge et al. \citep{ge2023hyperbolic} and Ramasinghe et al.~\citep{ramasinghe2024accept} used hyperbolic contrastive learning to enhance semantic coherence. Unlike previous methods that use only hyperbolic distance or angle, we fuse Euclidean and hyperbolic similarities into a hybrid metric, which boosts weakly supervised REC performance and showcases a new way to apply hyperbolic geometry in representation learning.

==> sections/3_problem.tex <==
\vspace{-2mm}

\section{Task Definition}

\vspace{-3mm}
% WGREC aims to localize all image regions described by a given natural language expression. Given an image $I$ and an expression $T$, the goal is to predict a set of bounding boxes: $\mathcal{B}^* = \{b_i \mid i \in k\}$, where each box $b_i$ corresponds to a region in $I$ that matches the expression $T$. The number of targets $k$ can vary: it may be zero, one, or more.

% In our weakly supervised setting, we do not use bounding box annotations during training. Each training sample consists only of an image–text pair $(I, T)$, without knowing which regions match the expression. Unlike WREC, which assumes every expression refers to a specific object, WGREC allows for expressions that have no matching region. To address this, we introduce a binary label $v \in \{0,1\}$ for the training set, where $v = 0$ means no region in the image matches the expression, and $v = 1$ otherwise. This provides weak supervision to guide the model in learning to predict all matching regions. Our goal is to train a model that, using only these weak labels, can predict the complete set of referent boxes for inference.

The Weakly-Supervised Generalized Referring Expression Comprehension (WGREC) task aims to localize all image regions described by a given natural language expression using only weak supervision. Formally, given an image $I$ and an expression $T$, the goal is to predict a set of bounding boxes, $\mathcal{B}^* = \{b_i \mid i \in k\}$, where each box $b_i$ corresponds to a region in $I$ that matches the expression $T$. and the number of targets $k$ is variable (zero, one, or more). Critically, no bounding box annotations are used during training. Each sample consists only of an image--text pair $(I, T)$, without knowing which regions match the expression. Unlike WREC, which assumes every expression refers to a specific object, WGREC allows for expressions that have no matching region. To address this, we introduce a binary label $v \in \{0,1\}$ for the training set, where $v = 0$ means no region in the image matches the expression, and $v = 1$ otherwise. This provides weak supervision to guide the model in learning to predict all matching regions. Our goal is to train a model that, using only these weak labels, can predict the complete set of referent boxes for inference.



\vspace{1em} % Adds a little vertical space before the summary paragraph


==> sections/4_Method.tex <==
\vspace{-3mm}
\section{Method}
\vspace{-2mm}

% Weakly supervised SOTA REC methods~\citep{jin2023refclip, luo2024apl, cheng2025weakmcn} simplify the referring expression comprehension (REC) task by reducing it to an anchor–text matching problem. Specifically, they select the most relevant anchor from a predefined set $\mathcal{A}$ using:
% \begin{equation}
% a^* = \arg\max_{a \in \mathcal{A}} \phi(T, I, a),
% \label{RECTask}
% \end{equation}
% where $\phi(T, I, a)$ denotes the similarity between the expression $T$, the image $I$, and anchor $a$.
% \textit{However, this max-selection strategy inherently assumes a single referent, making it unsuitable for generalized referring expression comprehension (GREC), where the number of targets is unknow.} To address this, we propose LIHE (Linguistic Instance-Split Hyperbolic-Euclidean), a framework designed for weakly supervised GREC. As shown in Fig.~\ref{fig:network}, LIHE consists of a referential decoupling stage, which decomposes complex expressions into single-instance queries, and a referent grounding stage, which detects all matching regions. In addition, we introduce a HEMix similarity to enforce hierarchical relationships.
%A natural alternative is to apply a threshold to filter anchors based on their similarity scores. Yet, our experimental analysis reveals the limitations of this approach. As shown in Figure~\ref{Similarity_Score}, the second-best anchor in some samples exhibits higher similarity than the top-scoring anchors in others, rendering a universal threshold ineffective for consistent selection. This highlights the inadequacy of threshold-based selection under GREC conditions.

%In this section, we begin by formally defining the weakly supervised GREC task and highlighting the limitations of existing weakly supervised REC methods in adapting to this more general setting. Inspired by human cognitive mechanisms for understanding referring expressions, we propose a weakly supervised framework that decomposes the GREC task into two distinct stages: the perception stage and the grounding stage, each of which is described in detail. Finally, we provide a theoretical justification for our proposed hybrid similarity measure, which effectively integrates Euclidean and hyperbolic spaces to enhance the performance of one-stage weakly supervised REC models during the grounding stage.
% Given an image \( I \) and a natural-language referring expression \( T \), the GREC task aims to predict a variable-length set of bounding boxes:
% \begin{equation}
% \mathcal{B}^{*} = \{\,b_{1}^{*}, b_{2}^{*}, \dots, b_{k}^{*}\,\}
%                  = \mathcal{F}_{\theta}(I, T),
% \label{eq:b_optimal}
% \end{equation}

% where each bounding box \( b_{i}^{*} \) encloses one of the visual entities described by the textual expression \( T \). Note that \( k \geq 0 \), thus allowing GREC to handle cases of zero, one, or multiple target instances within the image.

% Under the proposed Weakly Supervised GREC setting, instance-level annotations are completely unavailable during training. Specifically, the training data comprises pairs \( (I, T) \) labeled only by a binary image-level validity flag \( v \):
% \[
% v = \text{Valid}(T, I) =
% \begin{cases}
% 1, & \text{if there exists at least one visual entity in } I \text{ described by } T,\\[6pt]
% 0, & \text{otherwise (no visual entity in } I \text{ matches } T\text{).}
% \end{cases}
% \]

% Under this supervision setting, no bounding boxes, segmentation masks, landmark annotations, or category labels are provided. The model must therefore learn solely from the binary validity label \( v \), which indicates the presence or absence of any referent corresponding to the input expression.

% \subsection{Limitations of Existing Weak REC Methods}
%WREC methods such as RefCLIP effectively simplify the task by reducing it to an anchor-text matching problem. Specifically, the anchor selection mechanism in methods like RefCLIP can be expressed as:
% \begin{equation}
% a^* = \arg\max_{a \in \mathcal{A}} \phi(T, I, a),
% \label{RECTask}
% \end{equation}
% where \( \phi(T, I, a) \) represents the similarity between the text expression \( T \), the image \( I \), and anchor \( a \) from the anchor set \( \mathcal{A} \).
% However, this max-selection strategy implicitly assumes that the number of referred objects is known in advance, making it unsuitable for Generalized Referring Expression Comprehension (GREC), where the number of targets is unknown. A natural alternative is to apply a threshold to filter anchors based on their similarity scores. Yet, our experimental analysis reveals the limitations of this approach. As shown in Figure~\ref{Similarity_Score}, the second-best anchor in some samples exhibits higher similarity than the top-scoring anchors in others, rendering a universal threshold ineffective for consistent selection. This highlights the inadequacy of threshold-based selection under GREC conditions.

% \begin{figure*}
%     \centering
%     \setlength{\abovecaptionskip}{6pt}   % 图像与 caption 之间的距离
%     \setlength{\belowcaptionskip}{1pt}  % caption 与正文之间的距离，负值表示更紧凑
%     \includegraphics[width=1.0\linewidth]{images/Similarity_Score.pdf}
%     \caption{We randomly select 100 samples from the dataset and visualize their similarity scores. From left to right: (1) the similarity scores of top-scoring anchors (dark blue dots), (2) the similarity scores of second-best anchors (light blue squares), and (3) an overlaid view combining both. The dashed vertical segments connect the top and second-best scores for each sample, illustrating that second-best anchors in many cases have higher similarity than top anchors in other samples.}
%     \label{Similarity_Score}
% \end{figure*}

% \subsection{Framework}
% When humans perform a GREC task, they typically perceive each visual entity in the image in relation to the given referring expression. If a visual entity satisfies the semantic conditions described in the expression, it is recognized as a valid target, and then humans draw a frame based on the boundaries of the visual entity. 
% Inspired by this cognitive process, we introduce a perception stage using a pre-trained VLLM that aims to mimic this perception behavior by decomposing the referring expression into shorter, semantically focused phrases that facilitate more accurate visual entity identification. Then in the grounding stage, these short phrases are taken as a new referring expression with the image fed into an efficient one-stage weakly supervised REC model to grounding the target. An overview of the full framework is illustrated in Figure~\ref{fig:network}.

% In this section, we introduce the \textbf{L}inguistic \textbf{I}nstance-Split \textbf{H}yperbolic-\textbf{E}uclidean (LIHE)  framework, specifically designed to address the two fundamental challenges of WGREC: \textbf{Cardinality Ambiguity} and \textbf{Hierarchical Representation Collapse}. As illustrated in Fig.~\ref{fig:network}, LIHE operates through a two-stage pipeline that systematically resolves ``how many'' referents exist before determining ``which ones'' to ground. In the \textbf{Referential Decoupling} stage, we tackle Cardinality Ambiguity by leveraging a pre-trained vision-language model (VLM) to decompose complex referring expressions $T$ into simpler, instance-specific sub-expressions, effectively transforming the multi-referent problem into multiple single-referent tasks. Subsequently, the \textbf{Referent Grounding} stage localizes each generated sub-expression using a contrastive learning paradigm enhanced by \textbf{HEMix}, our novel hybrid similarity module that prevents Hierarchical Representation Collapse. Unlike standard approaches that rely solely on Euclidean metrics, HEMix synergizes Euclidean and hyperbolic geometries to preserve semantic distinctions while maintaining fine-grained alignment capabilities, thereby enabling robust performance across variable cardinality scenarios with negligible computational overhead. The following subsections provide detailed exposition of each stage.

Extending WREC to WGREC is non-trivial and typically faces two major challenges: \textbf{(1) Cardinality Ambiguity}:  WREC methods such as RefCLIP simplify the task by reducing it to an anchor–text matching problem. Specifically, they select the most relevant anchor from a predefined set $\mathcal{A}$ using:
\begin{equation}
a^* = \arg\max_{a \in \mathcal{A}} \phi(T, I, a),
\label{RECTask}
\end{equation}
where $\phi(T, I, a)$ denotes the similarity between the expression $T$, the image $I$, and anchor $a$. However, this max-selection strategy inherently assumes a single referent, making it unsuitable for WGREC, where the number of targets is unknown. \textbf{(2) Hierarchical Representation
Collapse}: When a general expression $T$ (e.g., ``person'') refers to multiple distinct sub-categories (e.g., a ``man'' and a ``woman'') as shown in Fig.~\ref{heratical}, conventional contrastive learning in Euclidean space can conflate their representations. This blurs categorical boundaries and leads to a loss of semantic distinction.

To address these limitations, we propose \textbf{L}inguistic \textbf{I}nstance-Split \textbf{H}yperbolic-\textbf{E}uclidean (LIHE), a framework designed for WGREC. As shown in Fig.~\ref{fig:network}, LIHE consists of a \textit{Referential Decoupling} stage, which decomposes complex expressions into single-instance queries, and a \textit{Referent Grounding} stage, which detects all matching regions. In addition, we introduce a \textit{HEMix} similarity to explicitly preserve hierarchical relationships.

\vspace{-1mm}
\subsection{Referential Decoupling}
\vspace{-1mm}
In the context of WGREC, referring expressions often correspond to multiple visual entities. To address this, we reformulate the task by decomposing a multi-target expression into a set of single-target sub-expressions, allowing each referent to be localized independently and utilize the capabilities of VLM~\citep{qwen2.5-VL} to judge whether the target exists. This strategy simplifies the multi-instance grounding problem and makes it more tractable under weak supervision.

We leverage the perceptual capabilities of large vision-language models (VLMs)~\citep{qwen2.5-VL}, which, although do not have grounding functions, exhibit strong visual understanding and language reasoning. Given an image $I$, a referring expression $T$, and a carefully designed prompt $P$, we input them into a VLM to obtain a set of simplified, instance-level expressions.
To exploit the in-context learning capability of the VLM, we design a four-part prompt paired with the input image to guide the VLM in decomposing the original referring expression:
(1) General instruction $\mathbf{P_G}$, describing the goal of splitting the expression into target-specific phrases;
(2) Output constraints $\mathbf{P_C}$, specifying the format of each phrase;
(3) In-context examples $\mathbf{P_E}$, providing annotated demonstrations to steer the VLM toward the desired behavior;
(4) Input query $\mathbf{P_Q}$, which contains original referring expression together with explicit instructions;
(5) Raw Image $\mathbf{I}$.
Decomposition is formulated as
\begin{equation}
K,\mathcal{T}_{\text{D}} = \text{VLM}(\mathbf{P_G},\, \mathbf{P_C},\, \mathbf{P_E},\, \mathbf{P_Q},\, \mathbf{I}),
% \mathcal{O}_{\text{D}} = \{\,K,\; t_0,\,t_1,\dots,t_{k-1}\,\}
\end{equation}
where $K$ is the number of targets and $\mathcal{T}_{\text{D}} = \{ t_1, t_2, \dots, t_k \}$ is the set of sub-expressions generated by the model, each describing a distinct visual entity potentially present in the image. The prompts $\mathbf{P}$ guide the model to rewrite the original expression into concise, non-overlapping descriptions of individual targets, using brief instructions and a few examples. This decomposition mitigates issues such as irrelevance and ambiguity. 
Meanwhile, the prompt component $\mathbf{P_C}$ explicitly instructs the VLM to first output the number of target phrases \(K\) before listing them. 
This constraint helps mitigate common hallucination issues in VLMs, such as generating duplicate referring expressions for the same visual entity. 
When the VLM returns ($K = 0$), we interpret it as a no-target case, which naturally fits the open-ended setting of WGREC. More detailed prompt design, please see Appendix~\ref{Appendix:DetailedPromptDesign}.

% \mathcal{T}_{\text{D}} = \text{VLM}(I, T, P),
% To exploit the in-context learning capability of a Large Language Model (LLM), we design a five-part prompt paired with the input image to guide the LLM in decomposing the original referring expression:
% (1) General instruction $\mathbf{P_G}$, describing the goal of splitting the expression into target-specific phrases;
% (2) Output constraints $\mathbf{P_C}$, specifying the format of each phrase;
% (3) In-context examples $\mathbf{P_E}$, providing annotated demonstrations to steer the LLM toward the desired behavior;
% (4) Input query $\mathbf{P_Q}$, which contains the original referring expression together with explicit instructions;
% (5) Visual tokens $\mathbf{V}$, extracted from the image by a pre-trained Vision Transformer (ViT) and supplied to the LLM to ground the textual cues.
% The decomposition is formulated as
% \begin{equation}
% \mathcal{O}_{\text{D}} = \{\,K,\; t_0,\,t_1,\dots,t_{k-1}\,\}
% = \text{LLM}(\mathbf{P_G},\, \mathbf{P_C},\, \mathbf{P_E},\, \mathbf{P_Q},\, \mathbf{V})
% \end{equation}

% where \(K\) is the number declared by the LLM and \(k\) is the actual count of generated phrases \(\{t_i\}\).  
% The prompt component \(P_C\) forces the LLM to output \(K\) before listing the phrases, which helps mitigate the hallucination effect of LLM, such as generating duplicate referring expressions for the same visual entity. In practice, \(k\) may differ from the declared \(K\); hence we use the total number of generated short phrases in \(\mathcal{T}_{\text{D}}\), as the effective target count. A value of \(k = 0\) indicates that no visual entity in the image matches the referring expression, implying a no-target case.

\begin{figure*}
    \centering
    \vspace{-6mm}
    \includegraphics[width=1.0\linewidth]{images/Main_Structure.pdf}
    \caption{\textbf{The overall framework of LIHE}. (a). Referential Decoupling: VLM decomposed the referring expression into distinct short phrases for each target. (b). Referent Grounding: Each phrase is processed by a textual encoder, and the image by a visual encoder. Then the model filters anchors of low value and returns the best-matching one for bounding box prediction. The referent grounding stage is weakly supervised by the anchor-based contrastive loss.}
    \label{fig:network}
    \vspace{-5mm}
\end{figure*}

\subsection{Referent Grounding}
After the decoupling stage, each decomposed referring expression \(t\) corresponds to a matched visual entity in the image \(I\). Consequently, the task reduces to a conventional WREC problem, as defined in Eq.~\ref{RECTask}. Therefore, the referent grounding stage of our framework follows the structure and training strategy of previous WREC methods~\citep{jin2023refclip,luo2024apl,cheng2025weakmcn}, which have proven effective for WREC. Specifically, given an input image and a referring expression (the short phrases generated from the referential decoupling stage), the model uses a one-stage detector to extract visual feature maps, from which anchor features are obtained.
We retain only the anchors from the last feature map layer—based on the assumption that most target objects in referring datasets are of moderate to large size and further filter them by confidence, typically keeping the top 10\% of anchors.
Each remaining anchor is projected into a joint semantic space, alongside the corresponding text embedding. The similarity between each anchor and the phrase is then computed using a hybrid similarity metric, which combines Euclidean and Hyperbolic similarity scores. 
Formally, we adopt the contrastive learning objective of RefCLIP~\citep{jin2023refclip}, replacing its similarity function with our HEMix:
\begin{equation}
\label{constrastive}
\mathcal{L}_c = - \log \frac{\exp\big( \text{HEMix}(f_{a_0}^i, f_t^i)/\tau \big)}{
\sum\limits_{n=0}^{N} \sum\limits_{j=0}^{M} \mathbb{I}_{\neg (i=j \wedge n \neq 0)} \exp\big( \text{HEMix}(f_{a_n}^j, f_t^i)/\tau \big)}
\end{equation}
where $f_{a_0}^i$ is the positive anchor for $i$-th image, $f_t^i$ is the text embedding, $\tau$ is a temperature scalar, and HEMix denotes our proposed Euclidean-Hyperbolic hybrid similarity. This contrastive objective aligns the correct anchor-text pair while using both intra- and inter-image anchors as negatives. More details of HEMix formulation are provided in Sec.~\ref{sec:hybrid-sim}. Note that we filter the training dataset for the referent grounding stage by retaining only samples with validity flag \(v=1\) (i.e., at least one entity in \(I\) matches \(T\)). 

\subsection{HEMix}
\label{sec:hybrid-sim}


In previous WREC methods~\citep{jin2023refclip,luo2024apl,cheng2025weakmcn}, contrastive learning is typically driven by Euclidean similarity in a shared embedding space. However, this approach is limited in its ability to capture hierarchical semantics. For instance, as illustrated in Fig.~\ref{heratical}, a phrase like \textit{`left person'} may refer to both \textit{`left man'} and \textit{`left woman'} two visual entities in the image, which are semantically related but visually distinct. Euclidean similarity tends to cluster all such instances together, resulting in ambiguous localization.
\begin{figure*}
    \centering
    \setlength{\abovecaptionskip}{6pt}   % 图像与 caption 之间的距离
    \setlength{\belowcaptionskip}{1pt}  % caption 与正文之间的距离，负值表示更紧凑
    \includegraphics[width=1.0\linewidth]{images/heratical.pdf}
    \caption{A simple illustration of (a) Euclidean flatten space and (b) hyperbolic Lorentz manifold in 3-dimensional space~\citep{li2024hyperbolic}. In Euclidean space, all nodes occupy a single, undifferentiated hierarchy, so parent and child entities share the same geometric scale.
    In contrast, the negative curvature of hyperbolic space naturally organizes nodes into concentric hierarchies: parent nodes reside closer to the manifold’s apex, while their children are pushed farther outward, and different children at the same level are repelled from one another.}
    \label{heratical}
\end{figure*}
To better model semantic structure, we incorporate hyperbolic geometry using the Lorentz (hyperboloid) model. Hyperbolic spaces naturally embed hierarchical relationships: pulling a parent concept (e.g., \textit{`person'}) closer to the time axis increases angular separation among its children (e.g., \textit{`man'} and \textit{`woman'}), effectively preserving both generality and specificity. This aligns well with the hierarchical nature of referring expressions. More introduction and insights are in Appendix~\ref{Appendix:Hyperbolic Space}. 

For $D$-Dimension visual feature $f_v \in \mathbb{R}^{D}$ and text feature $f_t \in \mathbb{R}^{D}$, we use two types of similarity:

(1) \textbf{Euclidean similarity}: Same as refclip~\citep{jin2023refclip}, the similarity is calculated by
\begin{equation}
\text{Sim}_{\mathrm{E}}(f_v, f_t) = \langle f_v \mathbf{W}_{EV},\; f_t \mathbf{W}_{ET} \rangle,
\end{equation}
where $\mathbf{W}_{EV}$ and $\mathbf{W}_{ET}$ are learnable linear mapping matrices, and $\langle \cdot, \cdot \rangle$ denotes the standard inner product in Euclidean space.

(2) \textbf{Hyperbolic similarity (Lorentz model)}: We first map features into hyperbolic space as spatial components of \(\tilde{f}_{v}, \tilde{f}_{t}\) in hyperbolic space:
\begin{equation}
\mathbf{z}_v = f_v \mathbf{W}_{HV} \in \mathbb{R}^{D}, \quad \mathbf{z}_t = f_t \mathbf{W}_{HT} \in \mathbb{R}^{D},
\end{equation}
where $\mathbf{W}_{HV}$ and $\mathbf{W}_{HT}$ are learnable linear projection matrices for hyperbolic space.
Here, instead of using exponential maps to embed into hyperbolic space in the paper before, which is prone to unstable gradients, we adopt a learnable linear projection for both branches. This ensures smooth training and better compatibility with contrastive objectives. 
In a hyperbolic space of curvature \(\kappa\), the calculation of hyperbolic similarity by the Lorentzian inner product is formulated as: 
\begin{equation}
\text{Sim}_{\mathrm{H}}(f_v, f_t) = \langle \tilde{f}_v, \tilde{f}_t \rangle_{\mathbb{H}} = -x_0^v x_0^t + \langle \mathbf{z}_v, \mathbf{z}_t \rangle,
\end{equation}
where the mapped feature vectors \(\tilde{f}_v = (x_0^v, \mathbf{z}_v) \in \mathbb{R}^{D+1},\quad
\tilde{f}_t = (x_0^t, \mathbf{z}_t) \in \mathbb{R}^{D+1}\) and the time components
\(x_0 = \smash[t]{\sqrt{\lVert \mathbf{z}\rVert^{2} + \kappa^{-1}}}\).
Due to the time component \(x_0\) being calculated from the spatial
component \(\mathbf{z}\), the feature vectors \(\tilde{f}\) satisfy
\(\langle \tilde{f}, \tilde{f} \rangle_{\mathbb{H}} = -\kappa^{-1}\).
Thus \(\tilde{f}\) represents a valid point in
\(
\mathbb{H}^n_\kappa = \{\mathbf{x} \in \mathbb{R}^{n+1} \mid
\langle \mathbf{x}, \mathbf{x} \rangle_\mathbb{H} = -\kappa^{-1},\; x_0 > 0\}
\)
and inherits the geometric properties of hyperbolic space.




 % ⟨x, x⟩H = −κ
% −1

% Then we lift them to Lorentz space by computing their time components using a constant negative curvature $\kappa < 0$:

% $$
% x_0 = \sqrt{\|\mathbf{z}\|^2 + \kappa^{-1}}.
% $$

% This yields Lorentz vectors:

% $$
% \tilde{f}_v = (x_0^v,\, \mathbf{z}_v), \quad \tilde{f}_t = (x_0^t,\, \mathbf{z}_t),
% $$

% and the Lorentzian inner product is defined as:

% $$
% \text{Sim}_{\mathrm{H}}(f_v, f_t) = \langle \tilde{f}_v, \tilde{f}_t \rangle_{\mathbb{H}} = -x_0^v x_0^t + \langle \mathbf{z}_v, \mathbf{z}_t \rangle.
% $$
% % Hyperbolic similarity (Lorentz model, compact form)

% We project visual and textual features into hyperbolic space through learnable linear maps  
% \( z_v = f_v W_{HV}, \; z_t = f_t W_{HT}. \)  
% Given a constant negative curvature \( \kappa<0 \), the time-like component is  
% \( x_0=\sqrt{\lVert z\rVert^{2}+\kappa^{-1}}. \)  
% The resulting Lorentz embeddings are \( \tilde f_v=(x_0^{v},z_v) \) and \( \tilde f_t=(x_0^{t},z_t) \).  
% Their hyperbolic similarity is the Lorentzian inner product  
% \[
% \operatorname{Sim}_{\mathrm H}(f_v,f_t)= -x_0^{v}x_0^{t}+\langle z_v,z_t\rangle .
% \]


(3) \textbf{HEMix similarity}: We define the final similarity as a weighted combination of the two:
\begin{equation}
\text{HEMix}(f_v, f_t) = (1 - \alpha) \, \text{Sim}_{\mathrm{E}}(f_v, f_t) + \alpha \, \text{Sim}_{\mathrm{H}}(f_v, f_t), \quad \alpha \in (0, 1).
\end{equation}
Euclidean space ($\kappa\!=\!0$ case) excels at \emph{local, flat} geometry; it preserves fine‑grained angular relationships that are crucial for pixel‑accurate localization.  
Lorentzian Hyperbolic space ($\kappa\!<\!0$ case) naturally embeds \emph{hierarchical} or long‑range semantics because geodesic distance grows exponentially~\citep{hyplorentz,ganea2018hyperbolic}, but its metric stretches neighborhoods close to the light cone, which can blur local details.  
Each geometry similarity (\(\text{Sim}_{\mathrm{E}}\) and \(\text{Sim}_{\mathrm{H}}\)) therefore introduces a different \emph{estimation error} with respect to the ideal but unknown similarity $\text{Sim}^{\star}$:
% \[
% \text{Sim}_{\mathrm{E}} = \text{Sim}^{\star} + \varepsilon_{\mathrm{E}}, 
% \qquad 
% \text{Sim}_{\mathrm{H}} = \text{Sim}^{\star} + \varepsilon_{\mathrm{H}}.
% \]
% Specifically, $\varepsilon_{\mathrm{E}}$ is large for hierarchical descriptions, while $\varepsilon_{\mathrm{H}}$ is large for micro‑spatial references. Meanwhile, the two errors are \emph{not} perfectly correlated, due to the characteristics of each space.
\[
\text{Sim}_{\mathrm{E}}=\text{Sim}^{\star}+b_{\mathrm{E}}+\varepsilon_{\mathrm{E}},\quad
\text{Sim}_{\mathrm{H}}=\text{Sim}^{\star}+b_{\mathrm{H}}+\varepsilon_{\mathrm{H}},
\]
where $b =\mathbb E[\text{Sim} -\text{Sim}^{\star}]$ denotes the \emph{bias} and $\varepsilon$ the zero‑mean random deviation. Specifically, $b_{\mathrm{E}}$ is large for hierarchical descriptions, while $b_{\mathrm{H}}$ is large for micro‑spatial references. The two errors are not perfectly correlated, due to the characteristics of each space.

\begin{proposition}[Variance reduction]
\label{prop:var-reduce}
Let $\sigma^{2}_{\mathrm{E}}\!=\!\operatorname{Var}[\varepsilon_{\mathrm{E}}]$,
$\sigma^{2}_{\mathrm{H}}\!=\!\operatorname{Var}[\varepsilon_{\mathrm{H}}]$
and $\rho\!=\!\operatorname{Corr}[\varepsilon_{\mathrm{E}},\varepsilon_{\mathrm{H}}]$.
If $\rho<1$, the mean‑squared error of the hybrid estimator
\begin{align*}
\operatorname{MSE}(\text{HEMix})
&=\mathbb E\bigl[(\text{HEMix}-\text{Sim}^{\star})^{2}\bigr]\\
&=((1-\alpha)b_{\mathrm{E}}+\alpha b_{\mathrm{H}})^{2}
\quad +(1-\alpha)^{2}\sigma_{\mathrm{E}}^{2}+\alpha^{2}\sigma_{\mathrm{H}}^{2}+2\alpha(1-\alpha)\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}},
\end{align*}
\text{attains its minimum at}
$\displaystyle
\alpha^{\star}=\frac{(\sigma_{\mathrm{E}}^{2}+\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}})+b_{\mathrm{E}}(b_{\mathrm{E}}-b_{\mathrm{H}})}{\sigma_{\mathrm{E}}^{2}+\sigma_{\mathrm{H}}^{2}-2\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}}+(b_{\mathrm{E}}-b_{\mathrm{H}})^{2}},
$
\text{and make} $\operatorname{MSE}(\text{HEMix})$ \text{satisfies}
\begin{equation}
    % \operatorname{MSE}(\text{HEMix})\!\leq\!\min\{\sigma^{2}_{\mathrm{E}},\sigma^{2}_{\mathrm{H}}\}.
    \operatorname{MSE}(\text{HEMix};\alpha^{\star})<\min\bigl\{\operatorname{MSE}(\text{Sim}_{\mathrm{E}}),\,\operatorname{MSE}(\text{Sim}_{\mathrm{H}})\bigr\}.
\end{equation}
\end{proposition}
% Please see the supplementary material for complete proof. Under the common assumption that the contrastive loss $\mathcal{L}\!\bigl(\sigma(S)\bigr)$ is Lipschitz\-continuous in $S$, a smaller mean\-squared error (MSE) yields a tighter generalization bound and therefore higher retrieval or localization accuracy. Because the inter\-space correlation $\rho$ is unknown, the best fusion weight $\alpha$ in~\eqref{eq:hybrid} is selected depending on the experiment. Equation~\eqref{eq:hybrid} integrates two complementary geometric views while aligning with the principle of \emph{spatial semantic consistency}: the ideal compatibility score $\text{Sim}^{\star}$ should remain invariant across spaces, but each space introduces its own approximation error due to its geometric bias. By selecting a proper $\alpha$, we leverage their complementary properties to form a better estimator that is closer to $\text{Sim}^{\star}$, ultimately improving generalization as demonstrated empirically in Section~\ref{Experiments}.
% In practice, we find that the hybrid similarity effectively balances local visual alignment and semantic hierarchy, resulting in more accurate and generalizable grounding, especially in open-world settings.
Please see the supplementary material for complete proof. Under the common assumption~\citep{huang2021towards,gouk2021regularisation,lei2023generalization} that the contrastive loss \(\mathcal{L}\!\bigl(\sigma(S)\bigr)\) is Lipschitz-continuous in its similarity argument \(S\), a lower MSE implies a tighter generalization bound, which translates into higher retrieval or localization accuracy. Due to \(\rho\) is unknown in practice, we select \(\alpha\) via experiment. Overall, HEMix unifies two complementary geometric inductive biases, local Euclidean precision and hyperbolic hierarchy, into a single estimator that better approximates \(\text{Sim}^{\star}\), as confirmed empirically in Sec.~\ref{Experiments}.

% \paragraph{Spatial semantic consistency revisited.} The ideal but unknown semantic compatibility $\text{Sim}^{\star}$ should be independent of the ambient geometry, yet the learned similarities are subject to space‑specific biases:
% \[
% \text{Sim}_{\mathrm{E}}=\text{Sim}^{\star}+b_{\mathrm{E}}+\varepsilon_{\mathrm{E}},\quad
% \text{Sim}_{\mathrm{H}}=\text{Sim}^{\star}+b_{\mathrm{H}}+\varepsilon_{\mathrm{H}},
% \]
% where $b_{\bullet}=\mathbb E[\text{Sim}_{\bullet}-\text{Sim}^{\star}]$ denotes the \emph{bias} and $\varepsilon_{\bullet}$ the zero‑mean random deviation.

% \paragraph{Why mixing helps with biased estimators.}
% The mean‑squared error (MSE) of the hybrid estimator relative to $\text{Sim}^{\star}$ is
% \begin{align}
% \operatorname{MSE}(\text{Sim}_{\mathrm{mix}})
% &=\mathbb E\bigl[(\text{Sim}_{\mathrm{mix}}-\text{Sim}^{\star})^{2}\bigr]\\
% &=((1-\alpha)b_{\mathrm{E}}+\alpha b_{\mathrm{H}})^{2}
% \quad +(1-\alpha)^{2}\sigma_{\mathrm{E}}^{2}+\alpha^{2}\sigma_{\mathrm{H}}^{2}+2\alpha(1-\alpha)\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}},
% \end{align}
% where $\sigma_{\bullet}^{2}=\operatorname{Var}[\varepsilon_{\bullet}]$ and $\rho=\operatorname{Corr}[\varepsilon_{\mathrm{E}},\varepsilon_{\mathrm{H}}]$. The first term captures joint bias, and the second line the combined variance.

% \begin{proposition}[Bias--variance trade‑off of the hybrid]
% \label{prop:bias-variance}
% If $(b_{\mathrm{E}},b_{\mathrm{H}})$ are not colinear with $(\sigma_{\mathrm{E}},\sigma_{\mathrm{H}})$ and $\rho<1$, there exists an $\alpha^{\star}\in(0,1)$ that minimises MSE and satisfies
% \begin{equation}
% \operatorname{MSE}(\text{Sim}_{\mathrm{mix}};\alpha^{\star})<\min\bigl\{\operatorname{MSE}(\text{Sim}_{\mathrm{E}}),\,\operatorname{MSE}(\text{Sim}_{\mathrm{H}})\bigr\}.
% \end{equation}
% \end{proposition}
% \emph{Sketch of proof.} The MSE is a quadratic function in $\alpha$ with positive curvature. Taking derivative yields a unique critical point
% \[
% \alpha^{\star}=\frac{(\sigma_{\mathrm{E}}^{2}+\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}})+b_{\mathrm{E}}(b_{\mathrm{E}}-b_{\mathrm{H}})}{\sigma_{\mathrm{E}}^{2}+\sigma_{\mathrm{H}}^{2}-2\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}}+(b_{\mathrm{E}}-b_{\mathrm{H}})^{2}},
% \]
% which lies in $(0,1)$ under the stated assumptions and lowers both bias and variance compared with either single‑space estimator. A detailed derivation is provided in the supplementary.

% \paragraph{Practical implication.} Even when neither space yields an unbiased similarity, their geometric biases differ. Learning $\alpha$ end‑to‑end lets the network exploit this complementarity, pushing the hybrid similarity closer to the geometry‑agnostic ideal $\text{Sim}^{\star}$ and translating to improved localization accuracy (Section~\ref{sec:experiments}).


% \paragraph{Definition.}

% Given an anchor visual feature \(f_v\) $\!\in\!\mathbb{R}^{d}$ and a language feature \(f_t\) $\!\in\!\mathbb{R}^{d}$,  
% we compute their Euclidean similarity
% \begin{equation}
% \text{Sim}_{\mathrm{E}}(f_v, f_t) \;=\;
% \langle f_v \textbf{\(\text{W}_{EV}\)},f_t\textbf{\(\text{W}_{ET}\)}\rangle_{\mathbb{E}} ,
% \end{equation}
% where \(\text{W}_{EV}\) and \(\text{W}_{ET}\) are Euclidean mapping metrics and their Hyperbolic similarity
% \begin{equation}
% \text{Sim}_{\mathrm{H}}(f_v,f_t)
% \;=\;
% \Bigl\langle
% \bigl(\sqrt{\kappa^{-1} +\|\mathbf{z}_{v}\|^{2}},\,\mathbf{z}_{v}\bigr),\;
% \bigl(\sqrt{\kappa^{-1} +\|\mathbf{z}_{t}\|^{2}},\,\mathbf{z}_{t}\bigr)
% \Bigr\rangle_{\mathbb{H}},
% \end{equation}
% where $\mathbf{z}_{v}\!= f_v \text{W}_{HV} $ and
% $\mathbf{z}_{t}\!= f_t \text{W}_{HT}$ are the \emph{spatial components}
% obtained from a learnable hyperbolic mapping metrics $W_{HV}$ and $W_{HT}\!\in\!\mathbb{R}^{d\times d}$,
% while the \emph{time component} is determined by the Lorentz manifold constraint and calculated from $\mathbf{z}_{v}$ and $\mathbf{z}_{t}$ by equation \ref{xtime}. Different from previous work using the exponential map to map the feature from Euclidean to Hyperbolic space, we use a learnable linear layer replacing it, because we observe the exponential map lead to an extremely high gradient and destroy the network parameters as shown in the experiment section.
% Eventually, the \textbf{hybrid similarity} is then defined as
% \begin{equation}
% \label{eq:hybrid}
% \text{Sim}_{\mathrm{mix}}(f_v,f_t)
% \;=\;(1-\alpha)\,\text{Sim}_{\mathrm{E}}(f_v,f_t)
%       \;+\;\alpha\,\text{Sim}_{\mathrm{H}}(f_v,f_t),
% \qquad
% \alpha\in(0,1).
% \end{equation}

% \paragraph{Why mix two geometries?}
% \begin{itemize}[leftmargin=12pt,itemsep=2pt]
%   \item \textbf{Euclidean space} ($\kappa\!=\!0$) excels at \emph{local, flat} geometry; it preserves fine‑grained angular relationships that are crucial for pixel‑accurate localization.  
%   \item \textbf{Lorentzian Hyperbolic space} ($\kappa\!<\!0$) naturally embeds \emph{hierarchical} or long‑range semantics because geodesic distance grows exponentially, but its metric stretches neighborhoods close to the light cone, which can blur local details.  
% \end{itemize}
% Each geometry therefore introduces a different \emph{estimation error} with respect to the true and ideal semantic compatibility $\text{Sim}^{\star}$:
% \[
% \text{Sim}_{\mathrm{E}} = \text{Sim}^{\star} + \varepsilon_{\mathrm{E}}, 
% \qquad 
% \text{Sim}_{\mathrm{H}} = \text{Sim}^{\star} + \varepsilon_{\mathrm{H}}.
% \]
% Empirically, $\varepsilon_{\mathrm{H}}$ is large for hierarchical descriptions, while $\varepsilon_{\mathrm{H}}$ is large for micro‑spatial references; the two errors are \emph{not} perfectly correlated, due to the characteristics of each space.

% \begin{proposition}[Variance reduction]
% \label{prop:var-reduce}
% Let $\sigma^{2}_{\mathrm{E}}\!=\!\operatorname{Var}[\varepsilon_{\mathrm{E}}]$,
% $\sigma^{2}_{\mathrm{H}}\!=\!\operatorname{Var}[\varepsilon_{\mathrm{H}}]$
% and $\rho\!=\!\operatorname{Corr}[\varepsilon_{\mathrm{E}},\varepsilon_{\mathrm{H}}]$.
% If $\rho<1$, the mean‑squared error of the hybrid estimator
% \[
% \operatorname{MSE}(\mathrm{Sim}_{\mathrm{mix}})=
% (1-\alpha)^{2}\sigma^{2}_{\mathrm{E}}+
% \alpha^{2}\sigma^{2}_{\mathrm{H}}+
% 2\alpha(1-\alpha)\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}}
% \]
% \text{attains its minimum at}
% $\displaystyle
% \alpha^{\star}=
% \dfrac{\sigma^{2}_{\mathrm{E}}-\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}}}
%       {\sigma^{2}_{\mathrm{E}}+\sigma^{2}_{\mathrm{H}}
%        -2\rho\sigma_{\mathrm{E}}\sigma_{\mathrm{H}}}\in(0,1)$
% \text{and make} $\operatorname{MSE}(\mathrm{Sim}_{\mathrm{mix}})$ \text{satisfies}
% \begin{equation}
%     \operatorname{MSE}(\mathrm{Sim}_{\mathrm{mix}})\!\leq\!\min\{\sigma^{2}_{\mathrm{E}},\sigma^{2}_{\mathrm{H}}\}.
% \end{equation}
% \end{proposition}

% \begin{proof}
% Expand $\operatorname{Var}[\text{Sim}_{\mathrm{mix}}-\text{Sim}^{\star}]$ to obtain the quadratic
% form above and differentiate w.r.t.\ $\alpha$.
% Because $\rho<1$, the stationary point lies strictly inside $(0,1)$ and the quadratic is positive‑definite, giving a unique global minimum that is strictly below both individual variances.
% \end{proof}
% Please see the supplementary material for a complete proof. Under the common assumption that the contrastive loss $\mathcal{L}\!\bigl(\sigma(S)\bigr)$ is Lipschitz\-continuous in $S$, a smaller mean\-squared error (MSE) yields a tighter generalization bound and therefore higher retrieval or localization accuracy. Because the inter\-space correlation $\rho$ is unknown, the best fusion weight $\alpha$ in~\eqref{eq:hybrid} is selected depending on the experiment. Equation~\eqref{eq:hybrid} integrates two complementary geometric views while aligning with the principle of \emph{spatial semantic consistency}: the ideal compatibility score $\text{Sim}^{\star}$ should remain invariant across spaces, but each space introduces its own approximation error due to its geometric bias. By selecting a proper $\alpha$, we leverage their complementary properties to form a better estimator that is closer to $\text{Sim}^{\star}$, ultimately improving generalization as demonstrated empirically in Section~\ref{Experiments}.


==> sections/5_expriments.tex <==
\vspace{-2mm}
\section{Experiments}
\label{Experiments}
\vspace{-1mm}
\subsection{Datasets and Metrics}
\vspace{-2mm}

We evaluate our proposed method on two benchmark datasets for the WGREC task: gRefCOCO~\citep{he2023grec} and Ref-ZOM~\citep{wang2025hierarchical}, both of which support expressions that may correspond to multiple or zero referents. Following prior works~\citep{he2023grec}, we adopt Precision@(F$_1$=1, IoU$\ge$0.5) and N-acc. as the main evaluation metrics. 
% These metrics are specifically designed to assess both instance-level precision and expression-level matching under the generalized setting. 
Precision@(F$_1$=1, IoU$\ge$0.5) computes the percentage of samples that have the F1 score of 1 with the IoU threshold set to 0.5 and N-acc. assesses the model’s proficiency in no-target identification.
Detailed explanations are provided in the Appendix~\ref{appendx:metrics}. 
To further validate the effectiveness and generalization ability of our proposed HEMix module, we also evaluate it on three widely-used WREC datasets: RefCOCO, RefCOCO+, and RefCOCOg. For these datasets, we follow the standard evaluation protocol using IoU@0.5, where a prediction is considered correct if the IoU between the predicted and ground-truth bounding box exceeds 0.5.
 

\begin{table}[t]
\setlength{\abovecaptionskip}{6pt}
\centering
\footnotesize
\caption{Comparison on the WGREC task. `$\dagger$' denotes these methods have been modified to generate multiple boxes following \citet{he2023grec}. 
`$^*$' denotes the model adapted for the WGREC task.}
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{1.5mm} % 调整列间距以适配新列
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|cc|cc|cc|cc}
\hline
\multirow{3}{*}{\textbf{Methods}} & \multirow{3}{*}{\textbf{Supervision}}  & \multicolumn{6}{c|}{\textbf{gRefCOCO}}& \multicolumn{2}{c}{\textbf{Ref-ZOM}} \\
\cline{3-8} \cline{9-10}
 &  &  \multicolumn{2}{c|}{val} & \multicolumn{2}{c|}{testA} & \multicolumn{2}{c|}{testB} & \multicolumn{2}{c}{val} \\
 & & Pr (\%) & N-acc.(\%) & Pr(\%) & N-acc.(\%) & Pr(\%) & N-acc.(\%) & Pr(\%) & N-acc.(\%) \\
\hline
MCN$^{\dag}$~\citep{luo2020multi}           & Fully & 28.0 & 30.6 & 32.3 & 32.0 & 26.8 & 30.3 & - & - \\
VLT$^{\dag}$~\citep{ding2021vision}           & Fully & 36.6 & 35.2 & 40.2 & 34.1 & 30.2 & 32.5 & - & -\\
MDETR$^{\dag}$~\citep{kamath2021mdetr}        & Fully & 42.7 & 36.3 & 50.0 & 34.5 & 36.5 & 31.0 & - & -\\
UNITEXT$^{\dag}$~\citep{yan2023universal}       & Fully  & 58.2 & 50.6 & 46.4 & 49.3 & 42.9 & 48.2 & - & -\\
Ferret-7B$^{*}$~\citep{you2023ferret}          & Fully & 54.8 & 48.9 & 49.5 & 45.2 & 43.5 & 43.8 & - & -\\
VistaLLM-7B~\citep{pramanick2024jack}          & Fully & 52.7 & 69.4 & - & - & - & - & - & -\\
VistaLLM-13B~\citep{pramanick2024jack}          & Fully  & 54.6 & 70.8 & - & - & - & - & - & -\\
RECANTFormer(5)~\citep{hemanthage2024recantformer} & Fully  & 57.73 &  52.70 & 57.82 & 53.38 & 49.49 & 54.53 & 56.69 &  88.24\\
RECANTFormer(10)~\citep{hemanthage2024recantformer}  & Fully &  55.10 & 52.73 & 55.07 & 53.07 & 48.01 & 54.81 & 59.78 &88.24\\
HieA2G$_\textrm{R101}$~\citep{wang2025hierarchical}  & Fully  & 67.8 & 60.3 & 66.0 & 60.1 & 56.5 & 56.0 & - & -\\
\hline
RefCLIP$^{*}$~\citep{jin2023refclip}           & Weakly &  17.85 & 0.0 & 18.23 & 0.0 & 21.89 & 0.0 & 35.78 & 0.0 \\
% \rowcolor{red}
    % LIHE with SimE & Weakly & 38.88 & 67.49 & 31.77 & 79.6 & 34.89 & 67.07 & - & 97.70 \\
\rowcolor{gray!15}
\textbf{LIHE} & \textbf{Weakly}  & \textbf{39.61} & \textbf{67.49} & \textbf{32.70} & \textbf{79.60} & \textbf{35.84} & \textbf{67.07} & \textbf{50.36} & \textbf{97.70} \\
\hline
\end{tabular}}}

\label{GREC}
\end{table}

\vspace{-1mm}
\subsection{Comparisons with State-of-the-art Methods}
\vspace{-2mm}
\paragraph{WGREC results.} 
As shown in Tab.~\ref{GREC}, LIHE achieves strong performance on the gRefCOCO dataset under the weakly supervised setting. 
Compared to other WREC baselines, RefCLIP~\citep{jin2023refclip}, our model significantly outperforms it across all splits. For instance, on the validation set, our method achieves 39.61\% grounding precision and 67.49\% normalized accuracy, while RefCLIP only obtains 17.85\% and lacks the capability to handle no-target cases. 
This performance gap clearly demonstrates that methods assuming a single target fail to generalize to WGREC, which involves multi-target and no-target scenarios. 
% While LIHE does not yet match the very top fully supervised Pr numbers, the comparison mixes supervision budgets: LIHE uses only image–text pairs plus a binary validity flag (no box annotations), avoiding expensive and labor-intensive instance-level annotations compared to fully supervised methods.  
Although fully supervised methods like HieA2G~\citep{wang2025hierarchical} and RECANTFormer~\citep{hemanthage2024recantformer} outperform our model in absolute metrics, our method remains competitive despite using only image-level supervision, and even surpasses earlier fully supervised baselines such as MCN~\citep{luo2020multi}, VLT~\citep{ding2021vision}, and MDETR~\citep{kamath2021mdetr}. 
Additionally, it is worth mentioning that our method can even accomplish unsupervised GREC tasks,
as shown in Appendix~\ref{Unsupervised Schema}.
\vspace{-3mm}


\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2mm}
\caption{Performance of our methods on RefCOCO, RefCOCO+ and RefCOCOg datasets. `*' indicates results reproduced under identical settings.}
\resizebox{0.9\textwidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|ccc|ccc|c}
\hline
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{Published on}} & 
\multicolumn{3}{c|}{\textbf{RefCOCO}} & 
\multicolumn{3}{c|}{\textbf{RefCOCO+}} & 
\multirow{1}{*}{\textbf{RefCOCOg}} \\
& & val & testA & testB & val & testA & testB & val \\
\hline
VC~\citep{niu2019variational}           & \textit{CVPR '18}    & -     & 32.68 & 27.22 & -     & 34.68 & 28.10 & 29.65 \\
ARN~\citep{liu2019adaptive}             & \textit{ICCV '19}    & 32.17 & 35.25 & 30.28 & 32.78 & 34.35 & 32.13 & 33.09 \\
IGN~\citep{zhang2020counterfactual}     & \textit{NeurIPS '20} & 34.78 & -     & -     & 36.91 & 36.91 & 35.46 & 34.92 \\
DTWREG~\citep{sun2021discriminative}    & \textit{TPAMI '21}   & 38.35 & 39.51 & 37.01 & 38.19 & 39.91 & 37.09 & 42.54 \\
\hline
RefCLIP*~\citep{jin2023refclip}   & \textit{CVPR '23}    & 59.88 & 58.44 & 56.91 & 40.11 & 40.01 & 38.63 & 47.87 \\
\textbf{RefCLIP*+HEMix} & - & \textbf{60.95} & \textbf{59.84} & \textbf{58.57} & \textbf{41.48} & \textbf{42.54}& \textbf{39.37} & \textbf{48.67} \\
\hline
APL*~\citep{luo2024apl}    & \textit{ECCV '24}    & 64.18 &  61.06 & 63.08 & 41.03 & 41.46 & 38.72 & 49.45 \\
\textbf{APL*+HEMix}  & -  & \textbf{65.71} & \textbf{62.67} & \textbf{64.04} & \textbf{42.13} & \textbf{42.98} & \textbf{40.70} & \textbf{50.88} \\
\hline
WeakMCN~\citep{cheng2025weakmcn}    & \textit{CVPR '25}    & 69.20 &  69.88 & 62.63 & 51.90 & 57.33 & 43.10 & 54.62 \\
\textbf{WeakMCN*+HEMix}  & -  & \textbf{70.44} & \textbf{71.59} & \textbf{63.22} & \textbf{52.61} & \textbf{58.14} & \textbf{44.43} & \textbf{55.60} \\
\hline
\end{tabular}
\label{tab:wrec-results}
}
\end{table}

\paragraph{WREC results.} 
We further evaluate the generalization ability of our hybrid similarity learning scheme on standard WREC benchmarks, including RefCOCO, RefCOCO+, and RefCOCOg. 
As shown in Tab.~\ref{tab:wrec-results}, integrating our proposed hybrid similarity module consistently improves existing baselines. 
For example, RefCLIP+HEMix surpasses vanilla RefCLIP on all splits (e.g., +1.71\% on RefCOCO testA, +1.15\% on RefCOCO+testA). 
Similarly, APL+HEMix yields consistent gains over APL~\citep{luo2024apl}, improving RefCOCOg by 1.43\% and RefCOCO+ testB by 1.98\% and WeakMCN+HEMix also improves the performance on three datasets. 
These results highlight the compatibility and plug-and-play nature of our hybrid similarity formulation. 
By combining Euclidean and Hyperbolic similarity measures, the model benefits from both local discriminative alignment and global semantic consistency, leading to better grounding performance across varying datasets and expression types.
\vspace{-2mm}
\subsection{Ablation Study}

\begin{table}[t]
\noindent
\footnotesize
\renewcommand{\arraystretch}{1.2}
\makebox[\textwidth][l]{ % ← 强制左对齐整组内容开始


\begin{minipage}[t]{0.5\textwidth}

\caption{Performance of different similarity methods in contrastive loss.}
\centering
\setlength{\tabcolsep}{1.2mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|ccc}
\hline
\multirow{2}{*}{\textbf{Similarity Method}} &\multicolumn{2}{c|}{\textbf{RefCOCO (WREC)}} &\multicolumn{3}{c}{\textbf{gRefCOCO (WGREC)}}\\

& testA & testB &val &testA &testB \\
\hline
$\mathrm{Sim}_\mathrm{E}$& 58.44  & 56.92 & 38.88	& 31.77	 &	34.89 \\
$\mathrm{Sim}_\mathrm{H}$& 58.94  & 57.72  & 39.58	 & 31.57  &	 36.88\\

 HEMix     & \textbf{59.84}  & \textbf{58.57} & \textbf{39.73}  & \textbf{32.19}  &  \textbf{37.22}\\

\hline
\end{tabular}
}
\label{ablation:sim}
\end{minipage}

\hspace{0.05\textwidth}

% \begin{minipage}[t]{0.4\textwidth}
% \caption{Performance of different hyperbolic mapping methods on RefCOCO.}
% \centering
% \setlength{\tabcolsep}{1.2mm}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|cc}
% \hline
% \multirow{2}{*}{Hyperbolic Mapping Method} &\multicolumn{2}{c}{RefCOCO}\\
% & testA & testB\\
% \hline

% Exponential Map & 54.16	& 53.78  \\
% Learnable Linear & \textbf{59.84}  & \textbf{58.57}  \\


% \hline
% \end{tabular}
% }
% \label{ablation:map}
% \end{minipage}

\begin{minipage}[t]{0.35\textwidth}
\centering
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{1.2mm}
\caption{Ablation study on the prompt design with N-acc. metrics}

\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\multirow{2}{*}{\textbf{Prompt design}} & \multicolumn{3}{c}{\textbf{gRefCOCO (WGREC)}} \\
              & val & testA & testB \\
\midrule
Without $P_E$ & 49.00 & 65.60 & 50.93 \\
$P^*$         & 68.10 & 76.66 & 68.26 \\
$P$           & 67.49 & 79.60 & 67.07 \\
\bottomrule
\end{tabular}
}
\label{ablation:prompt}
\end{minipage}
\vspace{-5mm}

% \begin{minipage}[t]{0.45\textwidth}
% \caption{Ablation on similarity, expmap, and dynamic $\alpha$ on RefCOCO.}
% \centering
% \setlength{\tabcolsep}{1.2mm}
% \begin{tabular}{c|c|c|c|cc}
% \hline
% \multirow{2}{*}{\(Sim_E\)} & \multirow{2}{*}{\(Sim_H\)} & \multirow{2}{*}{expmap} & \multirow{2}{*}{dyn. $\alpha$} & \multicolumn{2}{c}{RefCOCO} \\
%  & & & & testA & testB \\
% \hline
% \checkmark      &             &               &             & 58.44  & 56.92  \\
%                 &  \checkmark &               &             & 58.94  & 57.72  \\
% \rowcolor{gray!15}
%  \checkmark     &  \checkmark &               &             & 59.84  & 58.57  \\
%                 &  \checkmark &  \checkmark   &             & 51.33  & 52.62  \\
%  \checkmark     &  \checkmark & \checkmark    &             & 54.16	& 53.78  \\
%  \checkmark     & \checkmark  &               & \checkmark  & 57.84  & 56.78  \\
% \hline
% \end{tabular}
% \label{ablation1}
% \end{minipage}

% \hspace{0.05\textwidth}
% %
% \begin{minipage}[t]{0.45\textwidth}
% \caption{Ablation on similarity, explicit hierarchical constraints, on gRefCOCO.}
% \makeatletter\def\@captype{table}
% \centering
% \setlength{\tabcolsep}{1.5mm}
% \begin{tabular}{c|c|c|ccc}
% \hline
% \multirow{2}{*}{\(Sim_E\)} & \multirow{2}{*}{\(Sim_H\)} & \multirow{2}{*}{\makecell{Hier.\\Const.}} & \multicolumn{3}{c}{gRefCOCO} \\
%  & &  & val & testA & testB \\
% \hline
%  \checkmark     &               &               & 38.88	& 31.77	 &	34.89   \\
%                 &  \checkmark   &               & 39.58	 & 31.57  &	 36.88   \\
% \rowcolor{gray!15}
%  \checkmark     &  \checkmark   &               & 39.61  & 32.70  &  35.84   \\
%  \checkmark     &               & \checkmark    & 39.08  & 32.33  &	35.17 \\
%                 & \checkmark    & \checkmark    & 39.25  & 32.06  &	 36.03   \\
%  \checkmark     & \checkmark    & \checkmark    & 39.37	& 32.44	 &  36.62    \\
% \hline
% \end{tabular}
% \label{ablation2}
% \end{minipage}
}
\end{table}
\begin{table}[t]
\centering
\footnotesize
\caption{Cross-Dataset validation from GREC to REC benchmarks. In-Dataset denotes the model trained on the same dataset as the test.}
\vspace{-3mm}
\resizebox{0.75 \linewidth}{!}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|l|ccc|ccc|c}
\hline
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{Training Set}} & 
\multicolumn{3}{c|}{\textbf{RefCOCO}} & 
\multicolumn{3}{c|}{\textbf{RefCOCO+}} & 
\multirow{1}{*}{\textbf{RefCOCOg}} \\
& & val & testA & testB & val & testA & testB & val \\
\hline
RefCLIP & \multirow{2}{*}{In-Dataset} &59.88 &58.44 &56.91 &40.11 &40.01 &38.63 &47.87 \\
Ours &            & \textbf{60.95} & \textbf{59.84} & \textbf{58.57} & 41.48 & 42.54 & \textbf{39.37}  & 48.67     \\
% Ours & RefCOCO+           & -     & -     & -     &  & -     \\
% Ours & RefCOCOg           & -     & -     & -     & -     & -     & -      \\
\hline
RefCLIP    & \multirow{2}{*}{gRefCOCO}       & 47.62 & 46.83 & 48.53 & 38.25 & 38.91 & 38.00 & 43.73 \\
Ours    & & 54.34 & 55.79 & 51.38 & \textbf{42.04} & \textbf{43.22} & 38.84 & \textbf{49.14} \\
\hline
\end{tabular}
}
\label{ablation3}
\end{table}
\vspace{-2mm}
\begin{table}
\caption{Performance of different hyperbolic mapping methods on RefCOCO and WGREC.}
\vspace{-3mm}
\centering
% \setlength{\tabcolsep}{1.2mm}
\renewcommand{\arraystretch}{1.2}

\resizebox{0.75 \linewidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{Hyperbolic Mapping Method} & \multicolumn{3}{c|}{RefCOCO} & \multicolumn{3}{c}{WGREC}\\
& val & testA & testB & val & testA & testB\\
\hline
Exponential Map    & 55.02 & 54.16 & 53.78 & 38.65 & 31.44 & 34.37 \\
Learnable Linear   & \textbf{60.95} & \textbf{59.84} & \textbf{58.57} & \textbf{39.61} & \textbf{32.70} & \textbf{35.84} \\
\hline
\end{tabular}
}
\vspace{-3mm}
\label{ablation:mapall}
\end{table}

To validate the effectiveness of individual components in our framework, we conduct comprehensive ablation studies covering similarity modules, mapping strategies and cross-dataset validation. 
\vspace{-3mm}
\paragraph{Effect of Similarity Design in Contrastive Learning.}
We conduct an ablation study to assess the impact of different similarity functions in contrastive learning, as shown in Tab.~\ref{ablation:sim}. Overall, our proposed HEMix consistently outperforms standard Euclidean similarity ($\mathrm{Sim}_\mathrm{E}$, equivalent to Referent Grounding directly using RefCLIP), with average gains of 1.53\% on RefCOCO (WREC) and 0.90\% on gRefCOCO (WGREC), demonstrating its effectiveness across both tasks. When comparing $\mathrm{Sim}\mathrm{H}$ and $\mathrm{Sim}\mathrm{E}$, the improvement is more pronounced on WGREC than on WREC (+0.83\% vs. +0.65\%), and notably, $\mathrm{Sim}_\mathrm{H}$ achieves performance close to HEMix on WGREC, with only a 0.44\% gap on average. This suggests that hyperbolic similarity better supports the grounding of multiple semantically related referents, which is common in WGREC. One likely reason is that expressions in WGREC often correspond to multiple related but distinct instances, requiring a more structured representation space, an advantage naturally offered by hyperbolic geometry. These findings further confirm the suitability of hyperbolic space for modeling hierarchical semantics. Nevertheless, HEMix consistently outperforms both $\mathrm{Sim}\mathrm{E}$ and $\mathrm{Sim}\mathrm{H}$ across all datasets. Even in cases where $\mathrm{Sim}\mathrm{E}$ and $\mathrm{Sim}\mathrm{H}$ perform similarly (e.g., RefCOCO testA, gRefCOCO testA), HEMix achieves great improvements. This highlights the importance of incorporating both fine-grained and hierarchical information and demonstrates the overall superiority of our proposed HEMix.
% \vspace{-5mm}
\vspace{-3mm}

\paragraph{Ablation Study on Prompt design}
We conduct an ablation study on prompt design and use N-acc as metrics. The prompt $P$ contains $P_G$, $P_C$, $P_E$, $P_Q$ and $I$. Among them, $P_G$, $P_C$, $P_Q$, and $I$ are indispensable; the absence of any one would lead to unparseable VLM output and consequently task failure. Therefore, we present two variants: one with $P_E$ removed, and another, $P^*$, where the textual content is altered while preserving the semantic information of $P$.Removing $P_E$ led to some outputs not following the format well and reduced the model's understanding of the task, which in turn led to performance degradation. The performance of $P^*$ when changing the text content was similar to $P$, indicating the robustness of our method to prompts.
\vspace{-3mm}

\paragraph{Effect of Different Hyperbolic Mapping Designs.}
Prior works~\citep{hypfs,khrulkov2020hyperbolic,hypmeru}
typically adopt the exponential map to project features onto the hyperboloid manifold, preserving the mathematical correctness of hyperbolic embeddings. However, we observe that this mapping introduces steep gradients, which negatively affect training stability and optimization. As shown in Tab.~\ref{ablation:mapall}, replacing the exponential map with a learnable linear layer yields a substantial improvement of 5.24\% on RefCOCO and 1.23\% on gRefCOCO, indicating that a simpler, trainable mapping leads to better empirical performance in practice. To our best knowledge, only these two hyperbolic mapping schemes exist.
% \paragraph{Effect of Different Hyperbolic Mapping Designs.}
% Prior works~\citep{hyptxt1s,hyptxt2s,hyplorentz,hyppoincare,hier,hypvit,hypseg1,hypseg2,hypfs,khrulkov2020hyperbolic,hypmeru} typically adopt the exponential map to project features onto the hyperboloid manifold, preserving the mathematical correctness of hyperbolic embeddings. However, we observe that this mapping introduces steep gradients, which negatively affect training stability and optimization. As shown in Tab.~\ref{ablation:map} and more results in the Appendix, replacing the exponential map with a learnable linear layer yields a substantial improvement of 5.24\% on RefCOCO, indicating that a simpler, trainable mapping leads to better empirical performance in practice.
% \vspace{-4mm}
% \paragraph{Explicit $\textit{vs.}$ Implicit Hierarchical Constraints.}
% Tab.~\ref{ablation2} investigates whether explicitly adding hierarchical losses helps. In contrastive loss function (Eq.~\ref{constrastive}), similarity only involves the expression and the anchor vision feature, but we want to know whether it learns the whole hierarchy implicitly. To validate this, we add an extra explicit hierarchical constraint loss(details please see supplementary). As shown in Tab.~\ref{ablation2}, adding the explicit hierarchical constraint basically has the same performance, implying that through hyperbolic similarity model is able to learn Hierarchical Constraints Implicitly.
% We consider an additional supervision term:
% While such explicit constraints yield slight improvements in some cases (e.g., +0.45 on testA), the gains are marginal compared to the hybrid similarity alone. This implies that the hyperbolic similarity module can implicitly model hierarchical structures without requiring extra supervision.
% \begin{align*}
% \mathcal{L}_{\text{hier}} = \text{dist}_H(\text{cat}, \text{base\_ref}) + \text{dist}_H(\text{lan}, \text{base\_ref})
% \end{align*}
% \vspace{-5mm}
\vspace{-3mm}
\paragraph{Cross-Dataset Validation.}
To evaluate the robustness and generalization of our framework, we train the model on the gRefCOCO and test it on standard WREC benchmarks with single-target annotations. As shown in Tab.~\ref{ablation3}, our method consistently outperforms the single-target baseline RefCLIP across all test sets, despite being trained on the same gRefCOCO data. Compared to in-domain training, the cross-dataset setting yields even larger gains (e.g., +5.41\% $\textit{vs.}$ +0.80\% in RefCOCOg), further highlighting the superior transferability of our approach. Notably, our model even surpasses in-domain RefCLIP models on RefCOCO+ and RefCOCOg, demonstrating strong generalization across both task settings and dataset domains.


Furthermore, our more ablation study in Appendix~\ref{Appendix:More Ablation Studies} reveals several consistent trends across datasets. First, sweeping the hybrid weight $\alpha$ for HEMix produces a clear U-shaped curve with a robust sweet spot around $\alpha\!\in\![0.4,0.7]$; for example, RefCOCO testA peaks at $60.01\%$ when $\alpha{=}0.7$, while gRefCOCO testB reaches $36.44\%$ at $\alpha{=}0.9$ (Tab.~\ref{alphaab}). Second, adding an \emph{explicit} hierarchical constraint brings little to no average improvement over the \emph{implicit} structure already captured by HEMix (Tab.~\ref{hierarchicalconstrain}). Third, during referent grounding, excluding $v{=}0$ samples avoids degenerate contrastive updates and improves performance, while such cases are handled at inference by the referential decoupling stage, outputting ``0'' (Tab.~\ref{tab:refclip_v0}). 

\vspace{-4mm}
\subsection{Quantitative Analysis}
\vspace{-3mm}

\begin{figure}
    \centering
    \vspace{-4mm}
    \includegraphics[width=\linewidth]{images/visualize.pdf}
    \caption{Successful cases(green background) and failure cases(red background). The ground truth is denoted by red bounding boxes, whereas green bounding boxes denote the predictions.}
    \label{Quantitative}
    \vspace{-4mm}
\end{figure}
To further understand the behavior of our model in complex referring scenarios, we visualize representative success and failure cases from the gRefCOCO dataset in Fig.~\ref{Quantitative}. These examples highlight the strengths and current limitations of our framework.
\vspace{-3mm}

\paragraph{Success Cases.} As shown in Fig.~\ref{Quantitative}(A), our method demonstrates strong grounding ability across both multi-target and no-target expressions. For instance, in case (a), the expression includes multiple entities with spatial and appearance constraints, and our model is able to localize each person correctly despite heavy occlusion and crowd density. In (e), although the objects (donuts) are visually similar, our model grounds the correct ones by leveraging position cues. Moreover, our approach can successfully identify no-target cases (c) and (f). In (c), the phrase \textit{``the leftmost person wearing black uniform''} does not correspond to any entity in the image, and our model makes a correct no-target prediction. In (f), while the scene contains many people, none of them match the detailed attributes described in expression (\textit{``woman in red dress''}), and the model again avoids false positives.
\vspace{-3mm}
% \paragraph{Failure Cases.} Failure examples are shown in Fig.~\ref{Quantitative}(B), where we apply a strict evaluation criterion $\text{Pr@}(\text{F1} = 1,\, \text{IoU} \geq 0.5)$: a prediction is considered correct only if every predicted box matches a ground truth box one-to-one with an IoU $\geq$ 0.5. In (a), the phrase implies no valid target, but the model incorrectly grounds an entity, due to a limited understanding of the visual and textual semantics of VLM. As seen in (d), the model fails to localize fine-scale visual cues, such as small hands or blurred individuals. 
% In (b), the number of targets is predicted correctly, but all decomposed referring expressions are identical, due to VLM hallucinations. 
% (b) correctly predicts the number of targets, but all decomposed referring expressions collapse to the same label (``people''), reflecting a VLM hallucination. Although the model identifies four entities (two balls and two tennis rackets), class imbalance in training biases the decoder toward the high-frequency category, yielding four ``people" descriptions, consistent with prior reports of distribution-induced hallucination \citep{zhang2024knowledge, mckenna-etal-2023-sources, rohrbach-etal-2018-object, liang2025rbd}.
% In (c), although the short phrases from the referential decoupling stage are semantically valid and distinct, the grounding model struggles to segment accurate regions, resulting in overlap and missed detections.

\paragraph{Failure Cases.} Fig.~\ref{Quantitative}(B) presents typical failure cases. In (a), the expression implies no valid target, yet the model incorrectly grounds an entity, reflecting the limited semantic understanding of the VLM. In (b), the number of targets is predicted correctly, but all decomposed expressions collapse to the same label (``people''), caused by VLM hallucinations. This occurs despite correctly detecting four objects (two balls and two rackets); class imbalance biases the decoder toward the frequent category ``people,'' consistent with prior findings on distribution-induced hallucination~\citep{zhang2024knowledge,mckenna-etal-2023-sources,rohrbach-etal-2018-object,liang2025rbd}. In (c), although the decoupled phrases are semantically valid and distinct, the grounding stage fails to segment precise regions, leading to overlaps and missed detections. In (d), the model misses fine-scale visual cues, such as small hands or blurred individuals, demonstrating difficulty in handling subtle details.


==> sections/6_conclusion.tex <==
\vspace{-3mm}
\section{Conclusion}
\vspace{-3mm}

In this paper, we delve into the critical limitation of Weakly-Supervised Referring Expression Comprehension (WREC) task: the inability of existing methods to handle expressions corresponding to a variable number of targets. To address this, we introduce the Weakly-Supervised Generalized Referring Expression Comprehension (WGREC) task, a more realistic and challenging setting where an expression may refer to multiple, single, or no objects. We then propose LIHE, the first weakly-supervised framework designed for this generalized task. LIHE operates via a two-stage process: (1) Referential Decoupling, where a vision-language model (VLM) infers the number of potential referents and parses the expression into target-relevant sub-phrases, followed by (2) Referent Grounding, where the model enhanced by our novel hybrid similarity localizes each sub-phrase. This design leverages the semantic understanding of VLMs to resolve ambiguity and synergistically combines Euclidean and hyperbolic geometries to preserve hierarchical representations. Despite these strengths, experiments demonstrate that LIHE achieves state-of-the-art performance on both WGREC and WREC benchmarks, validating its robustness and generalization. One key limitation of LIHE is its reliance on VLMs, which limits inference speed ($\approx$2 FPS). Thus, LIHE is more suitable as a teacher model for generating pseudo-labels~\citep{diffusaliency} to supervise smaller, faster student models. In future work, we will explore student model design and lightweight VLM adaptation, as well as extend our hybrid similarity design to richer geometric formulations.



\section*{Reproducibility Statement}
All theoretical results are established under explicit conditions. Experimental details are given in Appendix~\ref{Appendix:Implementation Details}. The code and weights are available at \url{https://anonymous.4open.science/r/LIHE}.
\section*{Ethics Statement}
This work only uses publicly available datasets and does not involve human subjects or sensitive information. We identify no specific ethical concerns.

